Measuring Quantum Entropy

The entropy of a quantum system is a measure of its randomness, and has applications in measuring quantum entanglement. We study the problem of measuring the von Neumann entropy, $S(\rho)$, and R\'enyi entropy, $S_\alpha(\rho)$ of an unknown mixed quantum state $\rho$ in $d$ dimensions, given access to independent copies of $\rho$. We provide an algorithm with copy complexity $O(d^{2/\alpha})$ for estimating $S_\alpha(\rho)$ for $\alpha<1$, and copy complexity $O(d^{2})$ for estimating $S(\rho)$, and $S_\alpha(\rho)$ for non-integral $\alpha>1$. These bounds are at least quadratic in $d$, which is the order dependence on the number of copies required for learning the entire state $\rho$. For integral $\alpha>1$, on the other hand, we provide an algorithm for estimating $S_\alpha(\rho)$ with a sub-quadratic copy complexity of $O(d^{2-2/\alpha})$. We characterize the copy complexity for integral $\alpha>1$ up to constant factors by providing matching lower bounds. For other values of $\alpha$, and the von Neumann entropy, we show lower bounds on the algorithm that achieves the upper bound. This shows that we either need new algorithms for better upper bounds, or better lower bounds to tighten the results. For non-integral $\alpha$, and the von Neumann entropy, we consider the well known Empirical Young Diagram (EYD) algorithm, which is the analogue of empirical plug-in estimator in classical distribution estimation. As a corollary, we strengthen a lower bound on the copy complexity of the EYD algorithm for learning the maximally mixed state by showing that the lower bound holds with exponential probability (which was previously known to hold with a constant probability). For integral $\alpha>1$, we provide new concentration results of certain polynomials that arise in Kerov algebra of Young diagrams.

==> large-dims.tex <==
\subsection{Large $\dims$: $\dims>\frac1{\eps^{\renprm}}$}
In this case, we ask for the complexity of distinguishing whether the spectrum is $\eigv$, or $\eignuv$, which are given below:
\\
$\eigv = \Paren{\frac{1+\eps\dims^{1/\renprm}}{\dims}, \frac{1-\frac{\eps\dims^{1/\renprm}}{\dims-1}}{\dims},\ldots,\frac{1-\frac{\eps\dims^{1/\renprm}}{\dims-1}}{\dims}}$, \\
 $\eignuv =\Paren{\frac{1}{\dims},\ldots,\frac{1}{\dims}}$. 

We will prove the lower bound on the complexity of estimating $\rentprmmst{\renprm}{\mst}$ by proving the following two results. 

\begin{theorem}
\label{thm:large-dim} Suppose $\dims>\frac1{\eps^{\renprm}}$. 
Any algorithm that can distinguish between $\eigv$ and $\eignuv$ with probability at least $2/3$ requires at least $\Omega\Paren{\frac{\dims^{2-2/\renprm}}{\eps^{2}}}$ samples.
\end{theorem}

\begin{claim}
\label{clm:difference}
If $\dims>\frac1{\eps^{\renprm}}$, then 
\[
|\rent{\renprm}{\eigv}-\rent{\renprm}{\eignuv}|=\Theta(\eps^{\renprm})
\]	
\end{claim}
\begin{proof}
Computing the moments of $\eigv$, 
\begin{align}
\Map{\renprm}{\eigv} &= \frac1{\dims^{\renprm}}\Paren{\Paren{1+\eps\dims^{1/\renprm}}^{\renprm}+(\dims-1)\Paren{1-\frac{\eps\dims^{1/\renprm}}{\dims-1}}^{\renprm}}\nonumber\\
&\ge \frac1{\dims^{\renprm}}\Paren{d+\eps^{\renprm}\dims-\frac12\renprm\eps\dims^{1/\renprm}}\nonumber\\
& \ge\frac{d}{\dims^{\renprm}}\Paren{1+\frac13\eps^{\renprm}}\nonumber\\
& = \Map{\renprm}{\eignuv} \Paren{1+\frac13\eps^{\renprm}}\nonumber.
\end{align}
Taking logarithms and Taylor's series proves the lemma. 
\end{proof}

\begin{proof}[Proof of Theorem~\ref{thm:large-dim}]
The objective is to bound the $\chi^2$ distance between the SW distributions for the two states with $\ns$ copies. We use the following formula, derived in~\cite{OW16}. The result in this form was obtained from related results on Schur functions~\cite{OO, Ker}. 
\begin{lemma}[OW16]
\label{lem:chisq-uniform}
Let $x_1^\dims$ be such that $\sum x_i = 0$, and $x_i\ge-1$. Let $\eigv_x$ be the distribution with $\eigi{i}=(1+x_i)/\dims$. The all zero vector corresponds to the uniform distribution, which we denote by $\eigv_u$. Then the $\chi^2$ distance is equal to:
\[
\chisq{\eigv_x}{\eigv_u} =\sum_{\mu:0<|\mu|\le\dims}\frac{\schurlx{\mu}{x}^2}{\dims^{\overline{\absv\mu}}\dims^{|\mu|}}\ns^{\underline{|\mu|}}.
\] 
\end{lemma}

For us, the vector $x^d$ is $\dims\eigv-(1, \ldots, 1) = \Paren{{\eps\dims^{1/\renprm}}, \frac{\eps\dims^{1/\renprm}}{\dims-1},\ldots,\frac{\eps\dims^{1/\renprm}}{\dims-1}}$. Define $y^d = x^d/\eps= (\dims\eigv-(1, \ldots, 1))/\eps$. 

\noindent Using the fact that $s_\mu(x)$ is a symmetric homogeneous polynomial of degree $\absv{\mu}$, we obtain
\begin{align}
	\schurlx{\mu}{x^d} = \eps^{\absv{\mu}}\schurlx{\mu}{\yd}\label{eqn:schur-xy}.
\end{align}

We know that the number of different shapes of young tableaux with a given length $\ell$ is equal to the partition number of $\ell$. Moreover, the partition number $p(\ell)$ is less than $2^{3\sqrt \ell}$ for all $n$.\footnote{This is a simple, and potentially weak approximation of the partition number that follows from the Hardy-Ramanujam formula.} Therefore, it would suffice for us to consider only one shape for each length $\absv \mu$. This gives, 
\begin{align}
\chisq{\eigv_x}{\eigv_u}\le \sum_{\ind=1}^{\dims}\Brack{2^{3\sqrt \ind}\cdot\max_{\mu:\absv{\mu}=\ind} \frac{\schurlx{\mu}{\yd}^2}{\dims^{\overline{\ind}}\dims^{\ind}}\ns^{\underline{\ind}}\eps^{2\ind}}.\label{eqn:chi-sq-general}
\end{align}

We therefore consider any partition $\mu$ of $\ind$ and bound $\schurlx{\mu}{\yd}^2$. Let $\ydp$ be the vector of absolute values of $\yd$. Then, $\absv{\schurlx{\mu}{\yd}}\le\absv{\schurlx{\mu}{\ydp}}$. We will bound $\absv{\schurlx{\mu}{\ydp}}$.

The entries of $\ydp$ have a nice structure. There is only one element that is different from every other entry, and all other entries are identical. This allows us to use the Branching rule of Schur polynomials. 
\begin{lemma}[Branching Rule~\cite{2011-thingy}] The Schur polynomial $\schurlx{\mu}{z^d}$ can be decomposed as:
\begin{align}
\schurlx{\mu}{z^d} = \sum_{\lambda\prec \mu} z_d^{\absv{\mu} - \absv{\lambda}} \schurlx{\lambda}{z^{\dims-1}}\label{eqn:branching-rule}
\end{align}
where the summation is over all partitions $\lambda$ such that and $\mu_1\ge \lambda_1\ge\mu_2\ge\lambda_2\ge\mu_3\ge\ldots$,
\end{lemma}

Let $1^{r}$ be the vector of $r$ 1's. Applying this to $\ydp$, 
\begin{align}
\schurlx{\mu}{\ydp} = \sum_{\lambda\prec \mu} \Paren{\dims^{1/\renprm}}^{\absv{\mu}-\absv{\lambda}}\Paren{\frac{\dims^{1/\renprm}}{\dims-1}}^{|\lambda|}\schurlx{\lambda}{(1,\ldots,1)} = \sum_{\lambda\prec \mu} \dims^{\frac{\absv{\mu}}\renprm}\Paren{\frac1{\dims-1}}^{\absv{\lambda}}\schurlx{\lambda}{(1^d)}.
\end{align}

Now, $\schurlx{\lambda}{1^\dims}$ is the number of semistandard young tableaux with shape $\lambda$, and entries from $[\dims]$. It is known that 
\[
\schurlx{\lambda}{(1^{\dims})} = \prod_{1\leq i< j \leq n} \frac{\lambda_i - \lambda_j + j-i}{j-i}.
\]
However, we can trivially bound $\schurlx{\lambda}{(1^{\dims})}\le\dims^{\absv{\lambda}}$, the total number of ways of filling the young tableaux with entires from $[d]$ without any regard to ordering. 

\noindent We need one final definition.
\begin{definition}
For a partition $\mu$, let $\text{prec}(\mu)$ be the number of partitions $\lambda$ such that $\lambda\prec\mu$. 
\end{definition}

Therefore, 
\begin{align}
\schurlx{\mu}{y_+} 
&= \sum_{\lambda\prec \mu} \dims^{\frac{\absv{\mu}}\renprm}\Paren{\frac1{\dims-1}}^{\absv{\lambda}}\schurlx{\lambda}{(1^d)}\nonumber\\
&\le \text{prec}(\mu)\cdot 
\dims^{\frac{\absv{\mu}}\renprm}\Paren{\frac{\dims}{\dims-1}}^{\absv{\lambda}}\nonumber\\
&\le \text{prec}(\mu)\cdot 4\dims^{\frac{\absv{\mu}}\renprm},
\label{bound-schur-sp}
\end{align}
where in the last step we used that for $\dims\ge2$, $\Paren{\frac{\dims}{\dims-1}}^{\absv{\lambda}}\le \Paren{\frac{\dims}{\dims-1}}^{\dims}\le 4$. 


\begin{lemma}
\label{lem:prec}
Let $\absv{\mu}=\ind\le d$, then, 
\begin{align*}
\text{prec}(\mu) = \prod_{i=1}^{\infty}\Paren{\mu_i-\mu_{i+1}+1}< \ind^{\sqrt {2\ind}}
\end{align*}
\end{lemma}
\begin{proof}
The first equality is a simple counting argument. We therefore have to maximize the product. 
Let $\mltu_{i_1}>\mltu_{i_2}>\ldots>\mltu_{i_m}\ge1$ be all the distinct terms in $\mltu$.  If $\distinct=1$, the inequality is easy to show, else assume that $\mltu_{i_\distinct}\ge1$ Then, $\distinct(\distinct+1)/2\le \mltu_{i_1}+\ldots+\mltu_{i_\distinct}<\ind$, implying that $\distinct<\sqrt {2\ind}$. Moreover, $\mltu_{i_1}-\mltu_{i_\distinct}\le \absv{\mltu}=\ell.$
\begin{align}
\text{prec}(\mu)&\le \prod_{j=1}^{\distinct} \Paren{1+\mltu_{i_j}-\mltu_{i_{j+1}}}\nonumber \\
&\le \ind^\distinct\nonumber\\
&<\ind^{\sqrt {2\ind}},
\end{align}
where we have used that $\distinct>1$ implying that each term is at most $\ind$.
\end{proof}

Plugging~\eqref{bound-schur-sp}, and~\eqref{lem:prec} in~\eqref{eqn:chi-sq-general}, 
\begin{align}
\chisq{\eigv_x}{\eigv_u}&\le \sum_{\ind=1}^{\dims}\Brack{2^{3\sqrt \ind}\cdot\max_{\mu:\absv{\mu}=\ind} \frac{\schurlx{\mu}{\yd}^2}{\dims^{\overline{\ind}}\dims^{\ind}}\ns^{\underline{\ind}}\eps^{2\ind}}\\
&\le \sum_{\ind=1}^{\dims}\Brack{2^{3\sqrt \ind}\cdot \frac{\Paren{4\ind^{\sqrt {2\ind}}\cdot \dims^{\frac{\ind}\renprm}}^2}{\dims^{\overline{\ind}}\dims^{\ind}}\ns^{\underline{\ind}}\eps^{2\ind}}\nonumber\\
&\le \sum_{\ind=1}^{\dims}\Brack{\Paren{2\ind}^{3\sqrt \ind}\cdot \frac{\Paren{4\cdot \dims^{\frac{\ind}\renprm}}^2}{\dims^{\overline{\ind}}\dims^{\ind}}\ns^{\underline{\ind}}\eps^{2\ind}}\nonumber\\
&\le \sum_{\ind=1}^{\dims}16\Paren{2\ind}^{3\sqrt \ind}\cdot \Paren{\frac{\Paren{\dims^{\frac{1}\renprm}}^2\ns\eps^{2}}{\dims^{2}}}^{\ind}\nonumber\\
&= \sum_{\ind=1}^{\dims}16\Paren{2\ind}^{3\sqrt \ind}\cdot \Paren{\frac{\ns\eps^{2}}{\dims^{2-\frac2\renprm}}}^{\ind}.\nonumber
\end{align}
Finally using $\ind^{2\sqrt \ind}<2^{4\ind}= 16^\ind$, we get

\begin{align}
\chisq{\eigv_x}{\eigv_u} &= \sum_{\ind=1}^{\dims}16\cdot \Paren{\frac{16\ns\eps^{2}}{\dims^{2-\frac2\renprm}}}^{\ind}.\nonumber
\end{align}

Therefore, unless $n\ge\Omega\Paren{\frac{\dims^{2-\frac2{\renprm}}}{\eps^2}}$, the $\chi^2$ distance is small, proving the result.
\end{proof}



==> non-integral.tex <==
\section{Non Integral $\alpha$}

\subsection{$\alpha>1$}

In this section, we will prove the following:
\begin{theorem}
\label{thm:non-int-upper}
The empirical estimator of $\rentprmmst$ outputs an $\pm \eps$ estimate with  $O\Paren{\dims^2\Paren{\frac1{\eps^2}+\frac1{\eps^{2/\renprm}}}}$ samples.
\end{theorem}

We will use the following results to prove our result. 

\begin{lemma}
Let $\beta>1$, and $x> y>0$. Then, 
\[
x^{\beta}-y^{\beta}\le \Paren{x-y}\beta x^{\beta-1}.
\]
\end{lemma}
\begin{proof} 
By the mean value theorem, 
\begin{align}
\frac{x^{\beta}-y^{\beta}}{x-y}\le \max_{z\in[y,x]} \frac{d z^{\beta}}{dz}
\le \beta x^{\beta-1}. \nonumber
\end{align}
\end{proof}

\begin{lemma}
Suppose $Z$ is a random variable such that 
\begin{align}
\probof{\absv{Z}>t}<2e^{-t^2/8n},
\end{align}
then for any $\beta>1$, there is a constant $C_\beta$ such that
\[
\expectation{|Z|^\beta} < C_\beta n^{\beta/2}.
\]
\end{lemma}
\begin{proof}
\begin{align}
\expectation{|Z|^{\beta}} &= \int_{0}^{\infty} \probof{\absv{Z}^{\beta}>t^{\beta}}dt^{\beta}\nonumber\\
& = \int_{0}^{\infty}\beta t^{\beta-1} \probof{\absv{Z}>t}dt\nonumber\\
& \le \int_{0}^{\infty}2\beta t^{\beta-1} e^{-t^2/8n}dt.\nonumber
\end{align}
Using the transformation $u = t^2/8n$, we have $dt = \sqrt{8n/u}du/2$. This implies 
\begin{align}
\expectation{|Z|^{\beta}}
& \le \int_{0}^{\infty}\beta \Paren{\sqrt{8nu}}^{\beta-1} e^{-u}\sqrt{\frac{8n}u}du.\nonumber\\
& = \beta\Paren{{8n}}^{\beta/2}\int_{0}^{\infty}u^{\beta/2-1}  e^{-u}du\nonumber\\
& = \Paren{8^{\beta/2}\beta\Gamma(\frac\beta2)}{n}^{\beta/2},\nonumber
\end{align}
where $\Gamma(x)$ is the Gamma function. Choosing $C_\beta = 8^{\beta/2}\beta\Gamma(\frac\beta2)$ proves the lemma.
\end{proof}

We now prove the key component of our argument. 
\begin{lemma}
Let $\beta>1$, and further suppose that the sorted probabilities are $\eigi{i}$. Then there is a constant such that 
\[
\expectation{\absv{\lambi{i}^{\beta}-(\eigi{i}\ns)^\beta}}< C_{\beta}\cdot \Paren{n^{\beta/2} + \sqrt n(\eigi{i}\ns)^{\beta-1}}.
\]
\label{lem:diff-moment}
\end{lemma}

We now prove the copy complexity bound assuming this theorem. 

\begin{proof}[Proof of Theorem~\ref{thm:non-int-upper}]
Recall that $\ns = \sum \lambi{i}$. Define, 
\[
\Malamb{\renprm} \ed \sum_{i=1}^{\dims}\Paren{\frac{\lambi{i}}{\ns}}^{\renprm}.
\]
By Lemma~\ref{lem:diff-moment}, 
\begin{align}
\expectation{\absv{\Malamb{\renprm}-\Mapeigv{\renprm}}} 
& = \expectation{\frac1{\ns^{\renprm}}\absv{\sum_{i=1}^{\dims}\Paren{\Paren{\frac{\lambi{i}}{\ns}}^{\renprm}-\eigi{i}^\renprm}}}\nonumber\\
&\le \frac1{\ns^{\renprm}}\sum_{i=1}^{\dims}\expectation{\absv{\lambi{i}^{\renprm}-(\eigi{i}\ns)^\renprm}}\nonumber\\
&\le \frac{C_\renprm}{\ns^{\renprm}}\sum_{i=1}^{\dims} \Paren{\ns^{\renprm/2} + \sqrt \ns(\eigi{i}\ns)^{\renprm-1}} \nonumber\\
& = C_\renprm\Paren{\frac{\dims}{\ns^{\renprm/2}} + \frac1{\sqrt \ns}\sum_{i=1}^{\dims}\eigi{i}^{\renprm-1}} \nonumber\\
& = C_\renprm\Paren{\frac{\dims}{\ns^{\renprm/2}} + \frac{\Mapeigv{\renprm-1}}{\sqrt \ns}}. \label{eqn:non-int-bias}
\end{align}

Recall that for $\renprm>1$, we have $\Mapeigv{\renprm}\le \dims^{1-\renprm}$, and 
$\Mapeigv{\renprm-1}\le \dims\Mapeigv{\renprm}$. Substituting these two in~\eqref{eqn:non-int-bias}, we obtain
\begin{align}
\expectation{\absv{\Malamb{\renprm}-\Mapeigv{\renprm}}} 
& \le C_\renprm \Paren{\frac{\dims}{\ns^{\renprm/2}} + \frac{\Mapeigv{\renprm-1}}{\sqrt \ns}}\nonumber\\
& \le C_\renprm \Paren{\frac{\dims^{\renprm}\Mapeigv{\renprm}}{\ns^{\renprm/2}} + \frac{\dims\Mapeigv{\renprm}}{\sqrt \ns}}\nonumber\\
& \le C_\renprm \Paren{\frac{\dims^{\renprm}}{\ns^{\renprm/2}} + \frac{\dims}{\sqrt \ns}}\Mapeigv{\renprm}.\nonumber
\end{align}
By Markov's Inequality, 
\begin{align}
\probof{\absv{\Malamb{\renprm}-\Mapeigv{\renprm}}>\eps \Mapeigv{\renprm}}
&\le \frac{\expectation{\absv{\Malamb{\renprm}-\Mapeigv{\renprm}}}}{\eps\Mapeigv{\renprm}}\nonumber\\
& \le \frac{C_\renprm}{\eps}\Paren{\frac{\dims^{\renprm}}{\ns^{\renprm/2}} + \frac{\dims}{\sqrt \ns}}.
\end{align}
Therefore, when $\ns > C \dims^2\Paren{\frac1{\eps^2}+\frac1{\eps^{2/\renprm}}}$, the result follows.
\end{proof}






==> proof-of-lemma-15.tex <==

\begin{proof}[Proof of LEMMA for MOMENTS]
Theorem 1.4 of~\cite{OW17} states
\[
\eigvi{i}\ns -2\sqrt{\ns}\le\expectation{\lambi{i}} \le  \eigvi{i}\ns +2\sqrt{\ns}.
\]
Let
\begin{align}
\expectation{\lambi{i}} = \eigvi{i}\ns +\diffmean, \nonumber
\end{align}
where $\absv{\diffmean}\le 2\sqrt\ns$. 
Then, by the triangle inequality, 
\begin{align}
\expectation{\absv{\lambi{i}^{\beta}-(\eigi{i}\ns)^\beta}}
\le\ & \expectation{\absv{\lambi{i}^{\beta}-\Paren{\expectation{\lambi{i}}}^{\beta}}+\absv{\Paren{\expectation{\lambi{i}}}^{\beta}-(\eigi{i}\ns)^\beta}}\nonumber\\
=\ & \expectation{\absv{\lambi{i}^{\beta}-\Paren{\eigvi{i}\ns +\diffmean}^{\beta}}}+\absv{\Paren{\eigvi{i}\ns +\diffmean}^{\beta}-(\eigi{i}\ns)^\beta}.\nonumber
\end{align}
Consider the second term. By Lemma~\ref{lem:diff-moment}, and $|B|<2\sqrt\ns$, 
\begin{align}
\absv{\Paren{\eigvi{i}\ns +\diffmean}^{\beta}-(\eigi{i}\ns)^\beta} 
\le &\ \beta \cdot 2\sqrt\ns \Paren{\eigvi{i}\ns +2\sqrt\ns}^{\beta-1}\nonumber\\
< &\ \beta2^{\beta}\cdot  \Paren{\sqrt\ns\cdot (\eigvi{i}\ns)^{\beta-1}+\Paren{2\sqrt\ns}^{\beta}}.\nonumber
\end{align}
 Let $Z_i = \lambi{i}-\expectation{\lambi{i}} = \lambi{i}-\eigvi{i}\ns -\diffmean$. Then, $Z_i$ is a zero mean random variable. Recall from~\eqref{eqn:conc-lambi},
$\probof{\absv{Z_i}>t}\le e^{-t^2/2\ns}.$
Again applying Lemma~\ref{lem:diff-moment} to the first term, 
\begin{align}
\expectation{\absv{\lambi{i}^{\beta}-\Paren{\eigvi{i}\ns +\diffmean}^{\beta}}} 
= &\ \expectation{\absv{\Paren{Z_i+\eigvi{i}\ns +\diffmean}^{\beta}-\Paren{\eigvi{i}\ns +\diffmean}^{\beta}}} \nonumber\\
\le  & \ \beta\expectation{\absv{Z_i}\Paren{\absv{Z_i}+\eigvi{i}\ns +\absv{B}}^{\beta-1}}\nonumber\\
\le & \ \beta 3^{\beta-1} \expectation{\absv{Z_i}\Paren{\absv{Z_i}^{\beta-1}+(\eigvi{i}\ns)^{\beta-1} +\absv{B}^{\beta-1}}}\nonumber\\
= & \ \beta 3^{\beta-1} \expectation{\absv{Z_i}^{\beta}}+(\eigvi{i}\ns)^{\beta-1}\cdot\expectation{\absv{Z_i}} +\absv{B}^{\beta-1}\nonumber
\end{align}
Applying Lemma~\ref{lem:bounding-moments} to $Z_i$ gives the result. 
\end{proof}
